Scheduling Monotone Moldable Jobs in Linear Time

A moldable job is a job that can be executed on an arbitrary number of processors, and whose processing time depends on the number of processors allotted to it. A moldable job is monotone if its work doesn't decrease for an increasing number of allotted processors. We consider the problem of scheduling monotone moldable jobs to minimize the makespan. We argue that for certain compact input encodings a polynomial algorithm has a running time polynomial in n and log(m), where n is the number of jobs and m is the number of machines. We describe how monotony of jobs can be used to counteract the increased problem complexity that arises from compact encodings, and give tight bounds on the approximability of the problem with compact encoding: it is NP-hard to solve optimally, but admits a PTAS. The main focus of this work are efficient approximation algorithms. We describe different techniques to exploit the monotony of the jobs for better running times, and present a (3/2+{\epsilon})-approximate algorithm whose running time is polynomial in log(m) and 1/{\epsilon}, and only linear in the number n of jobs.

==> tikzlibraryboxes.code.tex <==
\RequirePackage{etoolbox}

\def\packing@x@min{0pt}
\def\packing@x@max{0pt}
\def\packing@x@diff{0pt}
\def\packing@x@lasti{min}
\def\packing@x@lastii{max}
\def\packing@y@min{0pt}
\def\packing@y@max{0pt}
\def\packing@y@diff{0pt}
\def\packing@y@lasti{min}
\def\packing@y@lastii{max}

\newcommand{\packing@setvar}[3]{% 1: x or y 2: min, max, diff 3: point
  \tikz@scan@one@point\pgfutil@firstofone #3\relax
  \csedef{packing@#1@#2}{\expandafter\the\csname pgf@#1\endcsname}%
  \ifcsstring{packing@#1@lasti}{#2}{%
  }{%
    \csletcs{packing@#1@lastii}{packing@#1@lasti}%
    \csedef{packing@#1@lasti}{#2}%
  }%
}

\pgfqkeys{/packing}{
  align left/.value required,
  align left/.code={\packing@setvar{x}{min}{#1}},
  align right/.value required,
  align right/.code={\packing@setvar{x}{max}{#1}},
  align bottom/.value required,
  align bottom/.code={\packing@setvar{y}{min}{#1}},
  align top/.value required,
  align top/.code={\packing@setvar{y}{max}{#1}},
  %
  width/.value required,
  width/.code={\packing@setvar{x}{diff}{(#1,0)}{x}},
  height/.value required,
  height/.code={\packing@setvar{y}{diff}{(0,#1)}},
  %
  x-min/.style={align left={(#1,0)}},
  x-max/.style={align right={(#1,0)}},
  y-min/.style={align bottom={(0,#1)}},
  y-max/.style={align top={(0,#1)}},
  %
  right of/.style={align left=(#1.east)},
  left of/.style={align right=(#1.west)},
  above of/.style={align bottom=(#1.north)},
  below of/.style={align top=(#1.south)},
}

\newcommand{\packing@ifhas}[4]{% If list #1 contains #2 execute #3 else #4
  \ifcsstring{packing@#1@lasti}{#2}{%
    #3%
  }{%
    \ifcsstring{packing@#1@lastii}{#2}{%
      #3%
    }{%
      #4%
    }%
  }%
}

% Calculate width/height if not set
\newcommand{\packing@calcmissing}[1]{%
  \packing@ifhas{#1}{diff}{%
    \packing@ifhas{#1}{min}{}{%
      \pgfmathparse{\csname packing@#1@max\endcsname-\csname packing@#1@diff\endcsname}%
      \csedef{packing@#1@min}{\pgfmathresult pt}%
    }%
  }{%
    \pgfmathparse{\csname packing@#1@max\endcsname-\csname packing@#1@min\endcsname}%
    \csedef{packing@#1@diff}{\pgfmathresult pt}%
  }
}

\tikzset{every pnode/.style={}}

\newcommand{\pnode}[3][]{%
    \pgfqkeys{/packing}{#2}
    \packing@calcmissing{x}
    \packing@calcmissing{y}
    \node[draw,every pnode,#1,anchor=south west,inner sep=0pt,outer sep=0pt,minimum width=\packing@x@diff,minimum height=\packing@y@diff]
      at (\packing@x@min,\packing@y@min) {#3};
}

\newcommand{\namedpnode}[4][]{%
    \pgfqkeys{/packing}{#2}
    \packing@calcmissing{x}
    \packing@calcmissing{y}
    \node[draw,every pnode,#1,anchor=south west,inner sep=0pt,outer sep=0pt,minimum width=\packing@x@diff,minimum height=\packing@y@diff]
      (#3) at (\packing@x@min,\packing@y@min) {#4};
}

\newcommand{\drawschedule}[2][]{%
	\draw[#1] (#2.north east)+(0,0.3) [dotted]-- +(0,1);
	\draw[#1] (#2.north east)+(0,0.3) -- (#2.south east);
	\draw[#1] (#2.south east) -- (#2.south west);
	\draw[#1] (#2.north west)+(0,0.3) -- (#2.south west);
	\draw[#1] (#2.north west)+(0,0.3) [dotted]-- +(0,1);
}

